Super-Mode OFDM with Index Modulation

Orthogonal frequency division multiplexing (OFDM) with index modulation (OFDM-IM) appears as a promising multi-carrier waveform candidate for beyond 5G due to its attractive advantages such as operational flexibility and ease of implementation. However, OFDM-IM may not be a proper choice for 5G services such as enhanced mobile broadband (eMBB) since achieving high data rates is challenging because of its null subcarriers. One solution to enhance the spectral efficiency of OFDM-IM is the employment of multiple distinguishable constellations (modes) by also exploiting its null subcarriers for data transmission. This paper proposes a novel IM technique called super-mode OFDM-IM (SuM-OFDM-IM), where mode activation patterns (MAPs) and subcarrier activation patterns (SAPs) are jointly selected and conventional data symbols are repetition coded over multiple subcarriers to achieve a diversity gain. For the proposed scheme, a low-complexity detector is designed, theoretical analyses are performed and a bit error rate (BER) upper bound is derived. The performance of the proposed system is also investigated through real-time experiments using a software-defined radio (SDR) based prototype. We show that SuM-OFDM-IM exhibits promising results in terms of spectral efficiency and error performance; thus, appears as a potential candidate for 5G and beyond communication systems.

==> bib.tex <==
@article{6G,
	title={What should {6G} be?},
	author={Dang, Shuping and Amin, Osama and Shihada, Basem and Alouini, Mohamed-Slim},
	journal={Nature Electronics},
	volume={3},
	number={1},
	pages={20--29},
	year={2020},
	publisher={Nature Publishing Group}
}


@article{lu2018compressed,
	title={Compressed-sensing-aided space-time frequency index modulation},
	author={Lu, Siyao and Hemadeh, Ibrahim A and El-Hajjar, Mohammed and Hanzo, Lajos},
	journal={IEEE Trans. Veh. Techol.},
	volume={67},
	number={7},
	pages={6259--6271},
	month={Jul.},
	year={2018},
	publisher={IEEE}
}

@ARTICLE{mao2018novel,
	author={T. {Mao} and Q. {Wang} and Z. {Wang} and S. {Chen}},
	journal={IEEE Commun. Surveys Tuts}, 
	title={Novel Index Modulation Techniques: A Survey}, 
	year={First Quarter 2019},
	volume={21},
	number={1},
	pages={315-348},}




@ARTICLE{OFDMIM,
  title={Orthogonal frequency division multiplexing with index modulation},
  author={Basar, Ertu{\u{g}}rul and Ayg{\"o}l{\"u}, {\"U}mit and Panay{\i}rc{\i}, Erdal and Poor, H Vincent},
  journal={IEEE Trans. Signal Process.},
  volume={61},
  number={22},
  pages={5536--5549},
  month={Nov.},
  year={2013},
  publisher={IEEE},}
  
  
  @article{IM,
  	title={Index modulation techniques for 5{G} wireless networks},
  	author={Basar, Ertugrul},
  	journal={IEEE Commun. Mag.},
  	volume={54},
  	number={7},
  	pages={168--175},
  	month={Jul.},
  	year={2016},
  	publisher={IEEE}
  }

@article{INTERLEAVE,
	title={{OFDM} with interleaved subcarrier-index modulation},
	author={Xiao, Yue and Wang, Shunshun and Dan, Lilin and Lei, Xia and Yang, Ping and Xiang, Wei},
	journal={IEEE Commun. Lett.},
	volume={18},
	number={8},
	pages={1447--1450},
	month={Aug.},
	year={2014},
	publisher={IEEE}
}


@article{CIOFDMIM,
	title={{OFDM} with index modulation using coordinate interleaving},
	author={Basar, Ertu{\u{g}}rul},
	journal={IEEE Wireless Commun. Lett.},
	volume={4},
	number={4},
	pages={381--384},
	month={Aug.},
	year={2015},
	publisher={IEEE}
}



@ARTICLE{OFDMSNM,
	author={A. M. {Jaradat} and J. M. {Hamamreh} and H. {Arslan}},
	journal={IEEE Wireless Commun. Lett.},
	title={{OFDM} With Subcarrier Number Modulation},
	month={Dec.},
	year={2018},
	volume={7},
	number={6},
	pages={914-917},
	keywords={error statistics;OFDM modulation;pulse width modulation;subcarrier number modulation;active subcarriers;OFDM subblock;specific information bits;index modulation;OFDM-IM;channel-dependent optimal subcarrier selection;orthogonal frequency division multiplexing;data transmission;bit error rate;pulse width modulation;OFDM;Modulation;Noise measurement;Receivers;Detectors;Transmitters;OFDM;subcarrier number modulation;index modulation;spectral efficiency;channel-dependent subcarrier selection},
	doi={10.1109/LWC.2018.2839624},
	ISSN={2162-2345},}



@article{LOWER,
	title={Lower Order Modulation Aided {BER} Reduction in {OFDM} With Index Modulation},
	author={Nambi, S Abhijith and Giridhar, K},
	journal={IEEE Commun. Lett.},
	volume={22},
	number={8},
	pages={1596--1599},
	month={Aug.},
	year={2018},
	publisher={IEEE}
}


@ARTICLE{DUAL,
	author={T. {Mao} and Z. {Wang} and Q. {Wang} and S. {Chen} and L. {Hanzo}},
	journal={IEEE Access},
	title={Dual-Mode Index Modulation Aided {OFDM}},
	month={Feb.},
	year={2017},
	volume={5},
	number={},
	pages={50-60},
	keywords={error statistics;maximum likelihood detection;OFDM modulation;dual-mode index modulation aided OFDM technique;orthogonal frequency division multiplexing;frequency domain subcarriers;bit error ratio;DM-OFDM;maximum likelihood detector;BER;reduced-complexity near optimal log-likelihood ratio-based detector;ML detector;pairwise error probability;Indexes;OFDM;Detectors;Phase shift keying;Throughput;Signal to noise ratio;Orthogonal frequency division multiplexing (OFDM);index modulation;index pattern;constellation;maximum likelihood detection;log-likelihood ratio based detection},
	doi={10.1109/ACCESS.2016.2601648},
	ISSN={2169-3536},
	month={},}



@ARTICLE{GDUAL,
	author={T. {Mao} and Q. {Wang} and Z. {Wang}},
	journal={IEEE Commun. Lett.},
	title={Generalized Dual-Mode Index Modulation Aided {OFDM}},
	year={2017},
	volume={21},
	number={4},
	pages={761-764},
	keywords={demodulation;error statistics;fading channels;maximum likelihood detection;multipath channels;OFDM modulation;dual-mode index modulation aided orthogonal frequency division multiplexing;generalized DM-OFDM;GDM-OFDM bit error rate performance degradation;subcarrier modulation;constellation mode;maximum-likelihood detector;reduced-complexity log-likelihood ratio detector;low signal-to-noise ratio;interleaving technique;demodulation;spectral efficiency enhancement;multipath fading channel;OFDM;Indexes;Modulation;Detectors;Fading channels;Niobium;Receivers;Orthogonal frequency division multiplexing (OFDM);index modulation;maximum likelihood detection;log-likelihood ratio based detection;interleaving technique},
	doi={10.1109/LCOMM.2016.2635634},
	ISSN={2373-7891},
	month={April},}


@article{MMOFDMIM,
	title={Multiple-mode orthogonal frequency division multiplexing with index modulation},
	author={Wen, Miaowen and Basar, Ertugrul and Li, Qiang and Zheng, Beixiong and Zhang, Meng},
	journal={IEEE Trans. on Commun.},
	volume={65},
	number={9},
	pages={3892--3906},
	month={Sep.},
	year={2017},
	publisher={IEEE}
}

@article{PRACT,
	title={Practical implementation of index modulation-based waveforms},
	author={Gokceli, Selahattin and Basar, Ertugrul and Wen, Miaowen and Kurt, Gunes Karabulut},
	journal={IEEE Access},
	volume={5},
	pages={25463--25473},
	year={2017},
	publisher={IEEE}
}


@article{GMM,
	title={Generalized multiple-mode {OFDM} with index modulation},
	author={Wen, Miaowen and Li, Qiang and Basar, Ertugrul and Zhang, Wensong},
	journal={IEEE Trans. Wireless Commun.},
	volume={17},
	number={10},
	pages={6531--6543},
	month={Oct.},
	year={2018},
	publisher={IEEE}
}

@article{DEMM,
	title={Diversity enhancing multiple-mode {OFDM} with index modulation},
	author={Li, Qiang and Wen, Miaowen and Basar, Ertugrul and Poor, H Vincent and Zheng, Beixiong and Chen, Fangjiong},
	journal={IEEE Trans. Commun.},
	volume={66},
	number={8},
	pages={3653--3666},
	month={Aug.},
	year={2018},
	publisher={IEEE}
}


@article{JOINT,
	title={Orthogonal Frequency Division Multiplexing With Joint Subblocks Index Modulation},
	author={Shi, Yuxin and Gao, Kai and Zhu, Jiang and Lu, Xinjin and Wang, Shilian},
	journal={IEEE Access},
	volume={7},
	pages={23930--23939},
	year={2019},
	publisher={IEEE}
}

@article{dang2017adaptive,
	title={Adaptive {OFDM} with index modulation for two-hop relay-assisted networks},
	author={Dang, Shuping and Coon, Justin P and Chen, Gaojie},
	journal={IEEE Trans. Wireless Commun.},
	volume={17},
	number={3},
	pages={1923--1936},
	month={Mar.},
	year={2018},
	publisher={IEEE}
}

@article{dang2018outage,
	title={Outage performance of two-hop {OFDM} with index modulation and multi-carrier relay selections},
	author={Dang, Shuping and Chen, Gaojie and Coon, Justin P},
	journal={IEEE Wireless Commun. Lett.},
	volume={7},
	number={6},
	pages={926--929},
	month={Dec.},
	year={2018},
	publisher={IEEE}
}

@article{basar2016multiple,
	title={On multiple-input multiple-output {OFDM} with index modulation for next generation wireless networks},
	author={Basar, Ertugrul},
	journal={IEEE Trans. Signal Process.},
	volume={64},
	number={15},
	pages={3868--3878},
	month={Aug.},
	year={2016},
	publisher={IEEE}
}

@article{zheng2017multiple,
	title={Multiple-input multiple-output {OFDM} with index modulation: Low-complexity detector design},
	author={Zheng, Beixiong and Wen, Miaowen and Basar, Ertugrul and Chen, Fangjiong},
	journal={IEEE Trans. Signal Process.},
	volume={65},
	number={11},
	pages={2758--2772},
	month={Jun.},
	year={2017},
	publisher={IEEE}
}

@article{ozturk2019multiple,
	title={Multiple-input multiple-output generalized frequency division multiplexing with index modulation},
	author={{\"O}zt{\"u}rk, Ersin and Basar, Ertugrul and {\c{C}}{\i}rpan, Hakan Ali},
	journal={Physical Communication},
	volume={34},
	pages={27--37},
	year={2019},
	publisher={Elsevier}
}



@INPROCEEDINGS{ma2017ofdm,
	author={Q. {Ma} and P. {Yang} and L. {Dan} and X. {He} and Y. {Xiao} and S. {Li}},
	booktitle={2017 IEEE 18th Int. Workshop on Signal Processing Advances in Wireless Commun. (SPAWC)},
	title={{OFDM-IM}-aided cooperative relaying protocol for cognitive radio networks},
	year={2017},
	volume={},
	number={},
	pages={1-5},
	keywords={cognitive radio;cooperative communication;decode and forward communication;error statistics;OFDM modulation;protocols;radiofrequency interference;relay networks (telecommunication);OFDM-IM-aided cooperative relaying protocol;overlay cognitive radio networks;transmission space;decode-and-forward relay;mutual interference;OFDM-based overlay CR networks;secondary networks;primary networks;two-phase orthogonal frequency division multiplexing-index modulation;finite-size constellations;bit error probability;information bits;primary user;secondary transmitter;index domain;signal constellation domain;secondary user;OFDM-IM technique;Protocols;OFDM;Indexes;Transmitters;Receivers;Modulation;Conferences;Cognitive radio (CR);cooperative relaying;decodes-and-forwards (DF);orthogonal frequency division multiplexing-index modulation (OFDM-IM)},
	doi={10.1109/SPAWC.2017.8227748},
	ISSN={1948-3252},
	month={July},}



@ARTICLE{li2019opportunistic,
	author={Q. {Li} and M. {Wen} and S. {Dang} and E. {Basar} and H. V. {Poor} and F. {Chen}},
	journal={IEEE Trans. Wireless Commun.},
	title={Opportunistic Spectrum Sharing Based on {OFDM} With Index Modulation},
	year={2019},
	volume={},
	number={},
	pages={1-1},
	keywords={OFDM;Wireless communication;Modulation;Relays;Signal to noise ratio;Bit error rate;Indexes;Amplify-and-forward relaying;cognitive radio;index modulation;OFDM;spectrum sharing},
	doi={10.1109/TWC.2019.2943159},
	ISSN={1558-2248},
	month={},}


@INPROCEEDINGS{bacsar2015optical,
	author={E. {Başar} and E. {Panayırcı}},
	booktitle={2015 4th International Workshop on Optical Wireless Communications (IWOW)},
	title={Optical {OFDM} with index modulation for visible light communications},
	year={2015},
	volume={},
	number={},
	pages={11-15},
	keywords={light emitting diodes;OFDM modulation;optical communication;optical OFDM;index modulation;visible light communications;optical orthogonal frequency division multiplexing;O-OFDM-IM;light emitting diodes;LED;photodetectors;active subcarriers;information bits;bipolar signals;log-likelihood ratio calculation;error peformance;OFDM;Adaptive optics;Noise measurement;Indexes;Wireless communication;Radio frequency;Light emitting diodes},
	doi={10.1109/IWOW.2015.7342256},
	ISSN={null},
	month={Sep.},}



@article{basar2017index,
	title={Index modulation techniques for next-generation wireless networks},
	author={Basar, Ertugrul and Wen, Miaowen and Mesleh, Raed and Di Renzo, Marco and Xiao, Yue and Haas, Harald},
	journal={IEEE Access},
	volume={5},
	pages={16693--16746},
	year={2017},
	publisher={IEEE}
}

@book{MIMOBOOK,
	title={MIMO-OFDM Wireless communications with MATLAB},
	author={Cho, Yong Soo and Kim, Jaekwon and Yang, Won Y and Kang, Chung G},
	year={2010},
	publisher={John Wiley \& Sons}
}


@inproceedings{arslan2003noise,
	title={Noise power and {SNR} estimation for {OFDM} based wireless communication systems},
	author={Arslan, H{\"u}seyin and Reddy, Sharath},
	booktitle={Proc. of 3rd IASTED Int. Conf. on Wireless Optical Commun. (WOC), Banff, Alberta, Canada},
	year={2003}
}

@ARTICLE{MOOSE,
	author={P. H. {Moose}},
	journal={IEEE Trans. Commun.},
	title={A technique for orthogonal frequency division multiplexing frequency offset correction},
	year={1994},
	volume={42},
	number={10},
	pages={2908-2914},
	keywords={frequency division multiplexing;maximum likelihood estimation;digital communication systems;parameter estimation;telecommunication channels;interference suppression;modulation;orthogonal frequency division multiplexing;frequency offset correction;digital communications;simulation;estimation error;OFDM signal;signal-to-interference ratios;intercarrier spacing;frequency offset estimation;repeated data symbol;maximum likelihood estimation;MLE algorithm;signal energy;intercarrier interference energy;symbol energy;initial acquisition;carrier spacing;modulation;multipath channels;OFDM;Frequency estimation;Maximum likelihood estimation;Interference;Digital communication;Computational modeling;Signal generators;Estimation error;Fading;Uncertainty},
	doi={10.1109/26.328961},
	ISSN={1558-0857},
	month={Oct},}

@ARTICLE{TDOFDM,
	author={J. {Zheng} and R. {Chen}},
	journal={IEEE Access},
	title={Achieving Transmit Diversity in {OFDM-IM} by Utilizing Multiple Signal Constellations},
	year={2017},
	volume={5},
	number={},
	pages={8978-8988},
	keywords={error statistics;OFDM modulation;probability;low-complexity log-likelihood ratio-based detector;average bit error probability;SC;TD;multicarrier modulation;orthogonal frequency division multiplexing;index modulation;transmit diversity achievement;multiple signal constellation;OFDM-IM;Indexes;OFDM;Constellation diagram;Detectors;Information rates;Simulation;OFDM;index modulation;transmit diversity;signal constellation},
	doi={10.1109/ACCESS.2017.2708718},
	ISSN={2169-3536},
	month={June},}

